Bs Physics at CDF and D0

Run II at the Tevatron has seen an explosion of results related to the Bs meson, ranging from tests of QCD models, to probes of electro-weak symmetry breaking, to direct searches for new physics effects. I will briefly summarize the CDF and D0 Bs-physics programs, describing the suitability of the detectors for doing this kind of physics, and pointing out how our knowledge of important quantities has improved through Run II measurements.

==> Makefile <==
#----------------------------------------------------
# Generic make file for LaTeX: requires GNU make
#
# This makefile provides four targets: dvi, pdf and clean.
# The default is "pdf".
# To make a dvi file, type "make dvi"
# To make a pdf file, type "make pdf" or simply "make".
# To remove all files generated by make, type "make clean".
#
# original from:
# Rouben Rostmaian <rostamian@umbc.edu>
# September 2002
# http://www.math.umbc.edu/~rouben/prosper/large_sample/Makefile
#
# Modifications
# 03-Apr-07  add LATEX and DVIPDF
#-------------------------------------------------------

TEXFILE	= evans_lathuile07_procs.tex
LATEX   = latex
DVIPDF  = dvipdfm

.PHONY: dvi pdf

pdf:	$(TEXFILE:.tex=.pdf)
dvi:	$(TEXFILE:.tex=.dvi)

%.dvi: %.tex
	${LATEX} $<
	latex_count=5 ;\
	while grep 'Rerun to get cross-references right' $(TEXFILE:.tex=.log) && [ $$latex_count -gt 0 ] ;\
		do \
			${LATEX} $< ;\
			latex_count=`expr $$latex_count - 1` ;\
		done

%.pdf: %.dvi
	${DVIPDF} -o $(<:.dvi=.pdf) $<

clean:
	@rm -f \
	$(TEXFILE:.tex=.aux) \
	$(TEXFILE:.tex=.log) \
	$(TEXFILE:.tex=.out) \
	$(TEXFILE:.tex=.dvi) \
	$(TEXFILE:.tex=.pdf)

# DO NOT DELETE



